T-Graphormer: Using Transformers for Spatiotemporal Forecasting

Spatiotemporal data is ubiquitous, and forecasting it has important applications in many domains. However, its complex cross-component dependencies and non-linear temporal dynamics can be challenging for traditional techniques. Existing methods address this by learning the two dimensions separately. Here, we introduce Temporal Graphormer (T-Graphormer), a Transformer-based approach capable of modelling spatiotemporal correlations simultaneously. By adding temporal encodings in the Graphormer architecture, each node attends to all other tokens within the graph sequence, enabling the model to learn rich spacetime patterns with minimal predefined inductive biases. We show the effectiveness of T-Graphormer on real-world traffic prediction benchmark datasets. Compared to state-of-the-art methods, T-Graphormer reduces root mean squared error (RMSE) and mean absolute percentage error (MAPE) by up to 20% and 10%.

==> figures/pretrain.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.475\linewidth}
        \centering
        \resizebox{\boxsize\linewidth}{!}{%
        \begin{tikzpicture}
            \definecolor{red}{RGB}{144,238,144}     % Red
            \definecolor{green}{RGB}{100,144,100}     % Green
            \definecolor{blue}{RGB}{0,128,255}     % Blue
            \definecolor{yellow}{RGB}{255,128,0}   % Yellow
            \definecolor{orange}{RGB}{255,128,100}   % Orange
            \begin{axis}[
                title={},
                width=\linewidth,
                xlabel={Seconds},
                ylabel={Mean Absolute Error},
                xmin=0, xmax=13200,
                ymin=3, ymax=8,  % Adjust the y-axis range according to your data
                xtick={0,2640,5280,7920,10560,13200},
                ytick={3,4,5,6,7,8},
                legend pos=north east,
                legend style={
                    nodes={scale=0.5, transform shape},
                    line width=.3pt,
                    mark size=.4pt
                },
                ymajorgrids=true,
                grid style=dashed,
            ]
            % PEMS-BAY (50 epochs)
            \addplot[
                color=orange,
                mark=o,
                mark size=1pt
                ]
                coordinates {(5737,4.752947391063045)(5874,4.992078921653191)(6011,4.408957370857177)(6148,4.1734915238404735)(6285,4.121675357222557)(6422,4.240865715805476)(6559,4.197666375506147)(6696,3.972069600758047)(6833,4.513904506854156)(6970,3.899063806175733)(7107,4.105762336877497)(7244,4.232274236053089)(7381,3.845282941464788)(7518,4.246630085658317)(7655,4.069631520980778)(7792,4.144554670451853)(7929,4.0849804119729205)(8066,4.023957103917323)(8203,4.202672500219893)(8340,4.109795983371577)(8477,4.513474437138327)(8614,3.875058121465704)(8751,4.229890731346106)(8888,4.510948687221716)(9025,4.28693832352183)(9162,3.65805767144503)(9299,3.7995092210699326)(9436,3.966028192280748)(9573,4.183531443414356)(9710,3.889640642095044)(9847,3.9026746658355904)(9984,4.155573953421804)(10121,3.862913741351532)(10258,3.94960099021321)(10395,3.7070473646571007)(10532,3.660689017876861)(10669,3.7874821072801184)(10806,3.873538436503019)(10943,3.947952445639976)(11080,3.6001809001682656)(11217,4.170960245292773)(11354,3.970975512582113)(11491,4.107116792555551)(11628,3.697503069498376)(11765,3.7503455899542666)(11902,3.898921796129408)(12039,3.916490932735049)(12176,3.8436650413514992)(12313,3.780801961890413)(12450,3.5960924022038965)
};
            
            \addplot[
                color=green,
                mark=o,
                mark size=1pt
                ]
                coordinates {(4537,4.548910438692388)(4674,3.917661739051969)(4811,4.303617507837295)(4948,4.227947780792819)(5085,3.902539921106301)(5222,4.419046013485466)(5359,3.800581073005484)(5496,3.769872233911339)(5633,4.106697170912488)(5770,4.080285020607794)(5907,3.892071560577916)(6044,4.141607773851464)(6181,4.081313669128848)(6318,4.2312020919085525)(6455,3.96884296843608)(6592,4.263497175405098)(6729,3.854471307926785)(6866,3.830206733301421)(7003,4.051407228611305)(7140,4.227968777460264)(7277,4.206426206688945)(7414,3.535916400627259)(7551,4.012487936943386)(7688,4.160613054483607)(7825,3.883230043744895)(7962,3.764297211216328)(8099,4.068033936727252)(8236,3.972726165454086)(8373,3.90289867807084)(8510,3.828686493966798)(8647,3.6548897232599207)(8784,3.65296461346568)(8921,3.521611778344089)(9058,3.900449340453668)(9195,3.646978478748178)(9332,3.537662078600342)(9469,3.4687741956038174)(9606,3.628737570004207)(9743,3.6125717803609567)(9880,3.45237781158779)(10017,3.52763166911813)(10154,3.553883481383428)(10291,3.556719313484451)(10428,3.4938739067352613)(10565,3.538468254242684)(10702,3.4507139081387805)(10839,3.537104016287409)(10976,3.5230845366517585)(11113,3.524705661077784)(11250,3.4449420414177405)
};

            \addplot[
                color=blue,
                mark=o,
                mark size=1pt
                ]
                coordinates {(3687,4.790514555972975)(3824,4.443932116562587)(3961,4.30674742438578)(4098,4.345900329952694)(4235,4.230382417154576)(4372,4.254587135678071)(4509,4.358956787830968)(4646,4.191299223471607)(4783,4.365903206352388)(4920,4.185524103336175)(5057,4.310194561627876)(5194,4.0746714316578325)(5331,4.034119063953512)(5468,4.229294476417007)(5605,4.148285877999684)(5742,4.083551761289519)(5879,4.01624453776281)(6016,4.048157003743)(6153,3.954130491533395)(6290,4.174651362772195)(6427,4.060588642841675)(6564,3.970920409779304)(6701,4.026705390325461)(6838,4.1142173328210605)(6975,4.019156235113531)(7112,3.8192332841099073)(7249,3.8293658022194337)(7386,3.9700821644113033)(7523,3.93707162029519)(7660,3.946787651657088)(7797,4.002806813094904)(7934,4.008849460196411)(8071,3.9609613130957095)(8208,4.029822264815394)(8345,3.95368107533622)(8482,3.81832782758365)(8619,3.871919371144167)(8756,3.985135208510698)(8893,3.860189222251979)(9030,3.877134855281753)(9167,4.052818876499676)(9304,3.8898283440367294)(9441,3.926190161172336)(9578,3.844250837632533)(9715,3.8847011560269538)(9852,3.855415052803947)(9989,4.064711519382093)(10126,3.9027897681971297)(10263,3.944385066491369)(10400,3.861462782811652)
};

            \addplot[
                color=yellow,
                mark=o,
                mark size=1pt
                ]
                coordinates {(137,5.795760276196438)(274,5.960056959660115)(411,6.1538952152357895)(548,6.1174854949708575)(685,5.275570920242049)(822,6.145466558957281)(959,6.343445551790576)(1096,5.274482975317879)(1233,5.62225058010701)(1370,7.248736287467182)(1507,4.813359450192025)(1644,4.439430425422284)(1781,4.208364495097999)(1918,3.993423177181769)(2055,4.15546742909823)(2192,3.7316412427984873)(2329,3.810840360815941)(2466,4.340172779258933)(2603,3.922387507552647)(2740,4.033288623228077)(2877,3.8181011167955456)(3014,3.894015374040736)(3151,4.0179014757763)(3288,3.7218859306771614)(3425,4.060228800940736)(3562,3.7224437784682087)(3699,3.8168100178563775)(3836,3.712550740615056)(3973,4.284761338385919)(4110,3.3253267515781464)(4247,3.8238311310768753)(4384,4.034659486755763)(4521,3.806328427503495)(4658,3.640299965566564)(4795,3.7112559880974274)(4932,3.4576132274450404)(5069,3.509341878128873)(5206,3.6001397158698154)(5343,3.900541826782348)(5480,3.5843677036029016)(5617,3.77852551202577)(5754,3.519356334995409)(5891,3.5267298483925167)(6028,3.426616494474219)(6165,3.4548463794951125)(6302,3.529368326302931)(6439,3.501678999348013)(6576,3.3285463101874653)(6713,3.4322644477235764)(6850,3.361087821437063)(6987,3.4025718542468675)(7124,3.3577209935375603)(7261,3.366854681642117)(7398,3.4989294733756404)(7535,3.284418207362608)(7672,3.300567273524912)(7809,3.458634544076902)(7946,3.239950350868716)(8083,3.453550124392958)(8220,3.2514845412311573)(8357,3.23844312724579)(8494,3.2472415296926607)(8631,3.327241613642774)(8768,3.241144948260354)(8905,3.264455254859874)(9042,3.1873734326093137)(9179,3.3216632902143504)(9316,3.259088819685488)(9453,3.267750395683868)(9590,3.2891381804300384)(9727,3.2345498389103144)(9864,3.229541613816101)(10001,3.290637345553733)(10138,3.2751772263801056)(10275,3.264219248380129)(10412,3.193037827825609)(10549,3.2212765562287142)(10686,3.1394498419826067)(10823,3.297069540551959)(10960,3.209845376953865)(11097,3.286147774014378)(11234,3.2870252463514005)(11371,3.203477339586243)(11508,3.271909892998601)(11645,3.2281050901102755)(11782,3.212316646384267)(11919,3.1890783939362617)(12056,3.205047798177628)(12193,3.227055309140167)(12330,3.1760100246032823)(12467,3.2658834466841244)(12604,3.2041958654516978)(12741,3.277989939586303)(12878,3.2184033702501904)(13015,3.216695977757885)(13152,3.223943966319001)(13289,3.277248716369167)(13426,3.239337629538517)(13563,3.236426728438133)(13700,3.1996575973440557)
};
            \legend{$0.3$, $0.5$, $0.7$, From scratch}               
            \end{axis}
        \end{tikzpicture}}
        \caption{Causal Prediction Layer}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.475\linewidth}
        \centering
        \resizebox{\boxsize\linewidth}{!}{%
        \begin{tikzpicture}
            \definecolor{red}{RGB}{144,238,144}     % Red
            \definecolor{green}{RGB}{100,144,100}     % Green
            \definecolor{blue}{RGB}{0,128,255}     % Blue
            \definecolor{yellow}{RGB}{255,128,0}   % Yellow
            \definecolor{orange}{RGB}{255,128,100}   % Orange
            
            \begin{axis}[
                title={},
                width=\linewidth,
                xlabel={Seconds},
                ylabel={Mean Absolute Error},
                xmin=0, xmax=13200,
                ymin=3, ymax=8,  % Adjust the y-axis range according to your data
                xtick={0,2640,5280,7920,10560,13200},
                ytick={3,4,5,6,7,8},
                legend pos=north east,
                legend style={
                    nodes={scale=0.5, transform shape},
                    line width=.3pt,
                    mark size=.4pt
                },
                ymajorgrids=true,
                grid style=dashed,
            ]
            
            \addplot[
                color=orange,
                mark=o,
                mark size=1pt
                ]
                coordinates {(5729,4.589613998038955)(5858,4.934515804670333)(5987,4.519445108919988)(6116,4.143718747126165)(6245,4.17543911257602)(6374,4.207978833297041)(6503,3.9559722330255833)(6632,4.05760529011958)(6761,4.139072856186915)(6890,3.8868684009126624)(7019,3.8138817143017234)(7148,3.819132299136336)(7277,3.8718370402919424)(7406,3.871900580771198)(7535,4.539062204535737)(7664,3.827561479044434)(7793,3.930177696462651)(7922,3.792930431938165)(8051,3.776675576500804)(8180,3.913190774654395)(8309,4.132762927431439)(8438,3.8250835277749418)(8567,4.03360073670536)(8696,3.873352301511565)(8825,3.8475431335750514)(8954,3.760111114998113)(9083,3.81101875446702)(9212,3.821517181791644)(9341,3.7834593838637818)(9470,3.922623754922893)(9599,3.920998749540788)(9728,3.802156133999369)(9857,3.88393099068133)(9986,3.967408111458209)(10115,3.686727459329207)(10244,3.749457940668146)(10373,3.752531874263398)(10502,3.793294233726946)(10631,3.8018781398379495)(10760,3.7263483623495306)(10889,3.837307191105716)(11018,3.7239479982320254)(11147,3.895762726708063)(11276,3.733415395439228)(11405,3.769320035183576)(11534,3.8053639088800857)(11663,3.9211761400617102)(11792,3.806747539438934)(11921,3.820963803622176)(12050,3.753067398731048)
};
            
            \addplot[
                color=green,
                mark=o,
                mark size=1pt
                ]
                coordinates {(4529,4.690944921695323)(4658,4.901546524428528)(4787,4.3689915452448425)(4916,4.0091971020196855)(5045,3.9611678261953953)(5174,4.012755632343937)(5303,3.878082693515293)(5432,3.985948359027992)(5561,3.9622279840834858)(5690,3.869134398573296)(5819,3.841245369728933)(5948,3.8336340992049984)(6077,3.83331163150093)(6206,3.821196259739243)(6335,4.159354608001135)(6464,3.740683514890304)(6593,3.807228424477557)(6722,3.719868931240428)(6851,3.895871202774764)(6980,3.792361043606858)(7109,3.75251118003208)(7238,3.6880385008701513)(7367,3.7708785839935888)(7496,3.705956850757944)(7625,3.6714041556806136)(7754,3.617435684035941)(7883,3.634188374278145)(8012,3.693495303992983)(8141,3.639682011308897)(8270,3.724408822282104)(8399,3.666694774531768)(8528,3.6624806830964154)(8657,3.724184320134189)(8786,3.762448063246453)(8915,3.5711512444453817)(9044,3.644399100945061)(9173,3.647494682202237)(9302,3.651550406920854)(9431,3.667509319143213)(9560,3.615964954980066)(9689,3.6685828558325975)(9818,3.615489273915224)(9947,3.6714271127777263)(10076,3.6003746322843586)(10205,3.6342416139380473)(10334,3.6371490618292346)(10463,3.6796780207768847)(10592,3.6438363658473176)(10721,3.652007279025443)(10850,3.615440491008111)
};
            \addplot[
                color=blue,
                mark=o,
                mark size=1pt
                ]
                coordinates {(3679,4.667702756151905)(3808,4.6495372039205005)(3937,4.248560211529833)(4066,4.21199362358148)(4195,4.148209879592618)(4324,4.115529359627306)(4453,4.282169403295058)(4582,4.177963169356895)(4711,4.078278564051595)(4840,4.122202771419886)(4969,4.040267654211547)(5098,4.063129427881964)(5227,4.0918538652743415)(5356,4.0869601557518696)(5485,4.239545814819182)(5614,4.144839308890471)(5743,4.04438294020316)(5872,4.065548290298364)(6001,3.90380362240232)(6130,4.069880207604511)(6259,4.004912315772097)(6388,3.9802513249723295)(6517,4.019601202112945)(6646,4.087531776633114)(6775,4.052049383268666)(6904,3.929070429541345)(7033,3.917730296652973)(7162,3.994186163222783)(7291,3.971998799692352)(7420,3.8990328531781926)(7549,3.967760909078904)(7678,3.951747270409784)(7807,3.8715484362382826)(7936,3.937878134051146)(8065,3.902821390410868)(8194,3.942526248810273)(8323,3.901596734722397)(8452,3.981650336850086)(8581,3.863617302101349)(8710,3.9045104068599503)(8839,3.91116117039765)(8968,3.905943309309431)(9097,3.910120391521916)(9226,3.88809353469166)(9355,3.956904007195904)(9484,3.898230338107934)(9613,3.925980311770549)(9742,3.875380149407086)(9871,3.949201707058003)(10000,3.9134293523765056)
};
            \addplot[
                color=yellow,
                mark=o,
                mark size=1pt
                ]
                coordinates {(129,5.79793665518932)(258,6.098682682543436)(387,6.57673357759611)(516,5.719036948788807)(645,5.529261329272222)(774,5.257685834132832)(903,6.11174453457243)(1032,4.08985442686913)(1161,3.983767500221207)(1290,4.336997358202412)(1419,4.145379588068854)(1548,5.0920708726430055)(1677,3.966731184270999)(1806,4.062322259079839)(1935,3.868895362483808)(2064,3.8776141388394008)(2193,3.9182202819795737)(2322,3.885148998458704)(2451,3.920634674091136)(2580,3.923549030250304)(2709,4.047168326054952)(2838,4.507654722170713)(2967,3.854498113657861)(3096,4.55925399665155)(3225,3.6776473945154695)(3354,3.649222396179233)(3483,4.70657852856512)(3612,3.63752091887938)(3741,4.371921384315415)(3870,3.4930363249199066)(3999,3.977651449312047)(4128,3.7888911972605737)(4257,3.6962460953933753)(4386,3.4514792027282657)(4515,3.4362046636823806)(4644,4.0297241198142695)(4773,3.440485005689106)(4902,3.3976255973766203)(5031,3.7663087751716375)(5160,3.505539067751058)(5289,3.5713944498049184)(5418,3.5025905541222646)(5547,3.445254399750173)(5676,3.5468576536905543)(5805,3.82942043055963)(5934,3.604708254354719)(6063,3.6318404262963786)(6192,3.4155206410344863)(6321,3.5465801993350143)(6450,3.698678425360889)(6579,3.720658159096699)(6708,3.4244711093613267)(6837,3.7604718634632426)(6966,3.3678922783104683)(7095,3.4683638156443903)(7224,3.4904419288874786)(7353,3.3588831735792284)(7482,3.432229202336449)(7611,3.533337810015845)(7740,3.453681416156763)(7869,3.5326335770165045)(7998,3.4551271061482622)(8127,3.4727930972639856)(8256,3.5671032174385946)(8385,3.5199237982960088)(8514,3.5529897694310573)(8643,3.56025562114648)(8772,3.3469223722632733)(8901,3.549789454104709)(9030,3.4471727666645267)(9159,3.4446813599206507)(9288,3.3524370110968005)(9417,3.386445397437141)(9546,3.278563680688668)(9675,3.431375457287253)(9804,3.3183930131049704)(9933,3.417859630546072)(10062,3.319938088519168)(10191,3.389920246996264)(10320,3.3604507224294835)(10449,3.4683615512379977)(10578,3.47139883857377)(10707,3.3114964562581384)(10836,3.339053318448469)(10965,3.335091810190406)(11094,3.333156996907092)(11223,3.3186023623343104)(11352,3.345986717371879)(11481,3.359632177034689)(11610,3.2998504370894874)(11739,3.42748115219994)(11868,3.2872638052294607)(11997,3.4213115866774717)(12126,3.274367378354421)(12255,3.293222252022753)(12384,3.325276692328261)(12513,3.413894050323761)(12642,3.344758453578732)(12771,3.3395194452055774)(12900,3.3051019450780177)
};
            \legend{$0.3$, $0.5$, $0.7$, From scratch}
            \end{axis}
        \end{tikzpicture}}
        \caption{Vanilla Prediction Layer}
    \end{subfigure}
    \caption{Performance comparison on the METR-LA traffic prediction dataset between masked self-supervised pre-training and training from scratch. Three masking ratios are evaluated for each prediction layer architecture. Each data point represents one epoch on the validation set. For pre-trained methods, the wall-clock time is calculated by adding the total pre-training time to the per-epoch training time (129 seconds for the vanilla prediction layer and 137 seconds for the causal prediction layer). Notably, higher masking ratios result in reduced pre-training time due to fewer tokens per batch. Since the METR-LA dataset is quite small, further experiments on larger datasets are needed to demonstrate the full pre-training potential.}
    \label{fig:pretrain_plot}
\end{figure}
